Chatting Makes Perfect: Chat-based Image Retrieval

Chats emerge as an effective user-friendly approach for information retrieval, and are successfully employed in many domains, such as customer service, healthcare, and finance. However, existing image retrieval approaches typically address the case of a single query-to-image round, and the use of chats for image retrieval has been mostly overlooked. In this work, we introduce ChatIR: a chat-based image retrieval system that engages in a conversation with the user to elicit information, in addition to an initial query, in order to clarify the user's search intent. Motivated by the capabilities of today's foundation models, we leverage Large Language Models to generate follow-up questions to an initial image description. These questions form a dialog with the user in order to retrieve the desired image from a large corpus. In this study, we explore the capabilities of such a system tested on a large dataset and reveal that engaging in a dialog yields significant gains in image retrieval. We start by building an evaluation pipeline from an existing manually generated dataset and explore different modules and training strategies for ChatIR. Our comparison includes strong baselines derived from related applications trained with Reinforcement Learning. Our system is capable of retrieving the target image from a pool of 50K images with over 78% success rate after 5 dialogue rounds, compared to 75% when questions are asked by humans, and 64% for a single shot text-to-image retrieval. Extensive evaluations reveal the strong capabilities and examine the limitations of CharIR under different settings. Project repository is available at https://github.com/levymsn/ChatIR.

==> chapters/task.tex <==
\section{ChatIR Task}
%\sout{In the Chat Image Retrieval (ChatIR) task the user is engaged in an interactive chat with the system in order to retrieve a desired image from a large image corpus. First, the user provides a textual description of the desired image, as done in Text-to-Image Retrieval. Next, a dialog ensues, where in each step, the user is prompted with a question asking for additional information about the desired image. The question and the user's answer (Q\&A) are appended to the dialog, thereby updating the search query. In practice, the chat may be terminated as soon as the desired image appears among the few top ranked retrieval results. Thus, ideally, each Q\&A round should be as informative as possible, narrowing down the set of candidates in the corpus, and getting closer to the target image.}\rnote{I think this is redundant. I am going to merge it with the next section}. Examples for chats and their retrievals candidates, produced by our model, are presented in \Cref{fig:retrieval_ex_5,fig:retrieval_ex_6}. 
Let us denote the ongoing dialog as $D_i:=(C,Q_1,A_1,...,Q_i,A_i)$, where $C$ is the initial text description (caption) of the target image, with $\{Q_k\}_{k=1}^{i}$ denoting the questions and $\{A_k\}_{k=1}^{i}$ their corresponding answers at round $i$.
Note that for $i=0$, $D_0 := (C)$ the input to $F$ is just the caption, \ie a special case of the Text-to-Image Retrieval task.

%The questions that arise in the context of the ChatIR task are:
% \begin{enumerate}
%     \item Is ChatIR indeed more effective than Text-to-Image retrieval; in other words, whether/how the retrieval accuracy improves as the dialog length increases beyond 0?
%     \item What is a ``good'' question to ask the user at each step of the process, and how to generate such questions?
%     \item How to measure/evaluate the effectiveness of different dialogue generation methods?
% \end{enumerate}
% \rnote{Refer to Fig. in Eval} Below, we present our testbed for exploring the ChatIR scenario, and in \Cref{sec:Evaluation} discuss the experiments that we conducted in an attempt to provide answers to the above questions.


